On the Effect of Triadic Closure on Network Segregation

The tendency for individuals to form social ties with others who are similar to themselves, known as homophily, is one of the most robust sociological principles. Since this phenomenon can lead to patterns of interactions that segregate people along different demographic dimensions, it can also lead to inequalities in access to information, resources, and opportunities. As we consider potential interventions that might alleviate the effects of segregation, we face the challenge that homophily constitutes a pervasive and organic force that is difficult to push back against. Designing effective interventions can therefore benefit from identifying counterbalancing social processes that might be harnessed to work in opposition to segregation. In this work, we show that triadic closure -- another common phenomenon that posits that individuals with a mutual connection are more likely to be connected to one another -- can be one such process. In doing so, we challenge a long-held belief that triadic closure and homophily work in tandem. By analyzing several fundamental network models using popular integration measures, we demonstrate the desegregating potential of triadic closure. We further empirically investigate this effect on real-world dynamic networks, surfacing observations that mirror our theoretical findings. We leverage these insights to discuss simple interventions that can help reduce segregation in settings that exhibit an interplay between triadic closure and homophily. We conclude with a discussion on qualitative implications for the design of interventions in settings where individuals arrive in an online fashion, and the designer can influence the initial set of connections.

==> sections/lemmas_and_theorems/dummy.tex <==
The change of integration from time $T+j-1$ to $T+j$ due to an intervention at time $T+i$ ($i < j$) is:
%
\begin{equation}
    \frac{1}{(N T)^2} \frac{K \alpha - 1}{K - 1} (-\Delta N_S^{(T+i)})
\end{equation}
%
where we simply found the difference of Equation~\ref{eq:interv_immediate} for $I=j$ and $I=j-1$. Now we can rewrite the rate of the change constraint from time $T+j-1$ to $T+j$ as:
%
\begin{equation}
    (-\Delta N_S^{(T+j)}) \le
    N T \Delta  - \sum_{i=1}^{j-1} \frac{N_F}{N T} \frac{K \alpha - 1}{K - 1} (-\Delta N_S^{(T+i)})
    .
\end{equation}
%

The objective function is also linear in $\{\Delta N_S^{(T+j)}\}$:
%
\begin{equation}
    f(T+I) = \frac{1}{N T} \sum_{i=1}^I \Big[1 + \frac{N_F}{N T}(I - i) \frac{K\alpha - 1}{K - 1} \Big] (-\Delta N_S^{(T + i)}) = \sum_{i=1}^I c_i (-\Delta N_S^{(T + i)})
\end{equation}
%
where $c_i$ is positive and decreasing in $i$. So, we have a linear programming problem. Let $-\Delta N_S^{(T+j)}=x_j$ ($j\in[I]$) be the optimum solution of the problem. We argue that for any $j\in[I]$, $x_j$ is the minimum of $N_S$ and $N T \Delta - \sum_{i=1}^{j-1} \frac{N_F}{N T} \frac{K \alpha - 1}{K - 1} x_i$. Otherwise, let $x_k$ be such a violation. It's easy to see $\exists \epsilon > 0$ such that
%
\begin{equation}
    -\Delta N_S^{(T+j)} = \bar{x}_j = \begin{cases}
        x_j + \epsilon & j=k \\
        x_j - \epsilon \frac{N_F}{N T} \frac{K \alpha - 1}{K - 1} & j > k \\
        x_j & j < k.
    \end{cases}
\end{equation}
%
satisfies the constraints. For large enough $\frac{I}{T}$, $\{\bar{x}_j\}$ will increase the objective function which is against the optimality of $\{x_j\}$. This proves the first part of the theorem. Intuitively, at each time step, the optimum solution greedily chooses $\Delta N_S^{(T+j)}$ as small as possible. 

Now if $N_S > N T \Delta$, according to the first part, $x_j = N T \Delta - \sum_{i=1}^{j-1} \frac{N_F}{N T} \frac{K \alpha - 1}{K - 1} x_i$ for all $j \in [I]$. This is a recursive equation for $x_j$. Let's define $y_j = \sum_{i=1}^j x_j$. The recursive definition for $y_j$ will be
%
\begin{equation}
    y_j - y_{j-1} = N T \Delta -\frac{N_F}{N T} \frac{K \alpha - 1}{K - 1} y_{j-1}
\end{equation}
%
and $y_1 = x_1 =  N T \Delta$. Taking $Z$-Transform from this recursive equation gives
%
\begin{equation}
    Y(z) = \frac{N T \Delta z^{-1}}{(1 - z^{-1})(1 - (1 - \frac{N_F}{N T} \frac{K \alpha - 1}{K - 1})z^{-1})}.
\end{equation}
%
By taking $Z^{-1}$-transform of $Y(Z)$ one can see
%
\begin{equation}
    y_j = \frac{N T \Delta}{\frac{N_F}{N T} \frac{K \alpha  - 1}{K - 1}} \Big[1 - (1 - \frac{N_F}{N T} \frac{K \alpha  - 1}{K - 1})^j \Big], \;\; j \ge 1
\end{equation}
%
and Equation~\ref{eq:optimum_interv} can be obtained by $\Delta N_S ^{(T+j)} = -x_j = y_{j-1} - y_j$.
